Deep Joint Rain Detection and Removal from a Single Image

In this paper, we address a rain removal problem from a single image, even in the presence of heavy rain and rain streak accumulation. Our core ideas lie in the new rain image models and a novel deep learning architecture. We first modify an existing model comprising a rain streak layer and a background layer, by adding a binary map that locates rain streak regions. Second, we create a new model consisting of a component representing rain streak accumulation (where individual streaks cannot be seen, and thus visually similar to mist or fog), and another component representing various shapes and directions of overlapping rain streaks, which usually happen in heavy rain. Based on the first model, we develop a multi-task deep learning architecture that learns the binary rain streak map, the appearance of rain streaks, and the clean background, which is our ultimate output. The additional binary map is critically beneficial, since its loss function can provide additional strong information to the network. To handle rain streak accumulation (again, a phenomenon visually similar to mist or fog) and various shapes and directions of overlapping rain streaks, we propose a recurrent rain detection and removal network that removes rain streaks and clears up the rain accumulation iteratively and progressively. In each recurrence of our method, a new contextualized dilated network is developed to exploit regional contextual information and outputs better representation for rain detection. The evaluation on real images, particularly on heavy rain, shows the effectiveness of our novel models and architecture, outperforming the state-of-the-art methods significantly. Our codes and data sets will be publicly available.

==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/001.tex <==

\def\height{2.6cm}
\def\name{001}
\def\namet{005}
\def\nameth{008}

\begin{figure*}[htbp]
	\begin{center}
		{ 	
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_001_GT.png}}
            \subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_001_in.png}}
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_ITRI_syn_removal_color_001_in.png}}	
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_DSC_syn_removal_001_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_LP_syn_removal_color_001_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_Joint-estimated-color-syn-removal-001_in.png}} \\ \vspace{-3mm}		
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/\namet_GT_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/\namet_in_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/ITRI_syn_removal_color_\namet_in_crop.png}}	
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/DSC_syn_removal_\namet_in_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/LP_syn_removal_color_\namet_in_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/Joint-estimated-color-syn-removal-\namet_in_crop.png}} \\ 
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_008_GT.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_ITRI_syn_removal_color_008_in.png}}	
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_DSC_syn_removal_008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_LP_syn_removal_color_008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_Joint-estimated-color-syn-removal-008_in.png}} \\			          
		} 
	\end{center}
	\vspace{-3mm}
	\caption{Subjective results of different methods on Rain12. From left to right: Ground truth, rain image, ID, DSC, LP and JORDER. From top to bottom: \textit{Image1} and \textit{Image8}.}
	\vspace{-4mm}
	
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/002.tex <==

\def\height{5cm}
\def\name{002}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/003.tex <==

\def\height{5cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/004.tex <==

\def\height{5cm}
\def\name{004}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/009.tex <==

\def\height{5cm}
\def\name{009}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/blur_case.tex <==

\def\height{5cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-001_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-002_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-003_in.png}}
			\\
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-004_in.png}}			
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-005_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-006_in.png}}
	        \\
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-007_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-009_in.png}}
			\\
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-010_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-011_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-012_in.png}}
		} 
	\end{center}
	\vspace{-2mm}
	\caption{Rain streak removal results on the synthesized blurred images. Blur kernel: Gaussian, whose range is $5\times5$ and blur level $2$.}
	\label{fig:blur_case}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/heavy.tex <==

\def\height{3.6cm}

\begin{figure}[htbp]
	\begin{center}
		{ 	
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/norain-152.png}}
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/rain-152.png}} \\
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-FT-removal-rain-152.png}}	
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-IEF-FT-removal-rain-152.png}}	
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/norain-115.png}}
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/rain-115.png}}
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-FT-removal-rain-115.png}}	
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-IEF-FT-removal-rain-115.png}}		          
		} 
	\end{center}
	\vspace{-3mm}
	\caption{The results of different methods on the testing image \textit{152} in \textit{Rain100H}.}
	\vspace{-5mm}
	\label{fig:heavy_cases_152}
\end{figure}
\vspace{-2mm}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/mist_case.tex <==

\def\height{5cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-001_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-002_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-003_in.png}}
			\\
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-004_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-005_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-006_in.png}}
	        \\
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-007_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-009_in.png}}
			\\			
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-010_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-011_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-012_in.png}}
		} 
	\end{center}
	\vspace{-5mm}
	\caption{Rain streak removal results on the synthesized mist images. Fixed transmission: 0.75. Atmospheric light: 0.75.  }
	\label{fig:mist_case}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/p002.tex <==

\def\height{3.7cm}
\def\name{p2}
\def\namet{p19}
\def\nameth{p11}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
			\includegraphics[height=\height,clip]{./Images/\name/GT_\name.jpg}}
			\subfigure{
				\includegraphics[height=\height,clip]{./Images/\namet/GT_\namet.jpg}}
			\subfigure{
				\includegraphics[height=\height,clip]{./Images/\nameth/GT_\nameth.jpg}}
		   \\	
	       \subfigure{
	       	\includegraphics[height=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}
	       \subfigure{
	       	\includegraphics[height=\height,clip]{./Images/\namet/DSC_real_removal_\namet.jpg}}
	       \subfigure{
	       	\includegraphics[height=\height,clip]{./Images/\nameth/DSC_real_removal_\nameth.jpg}}	       
	       \\ 			
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\namet/LP_real_removal_\namet.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\nameth/LP_real_removal_\nameth.jpg}}
           \\
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\name/Joint-estimated-color-Our-FT-removal-Joint-estimated-color-Our-FT-removal-p2.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\namet/Joint-estimated-color-Our-FT-removal-Joint-estimated-color-Our-FT-removal-p19.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\nameth/Joint-estimated-color-Our-FT-removal-Joint-estimated-color-Our-FT-removal-p11.jpg}}           
		} 
	\end{center}
	\vspace{-2mm}
	\caption{Subjective results of different methods on real images. From top to down: rain image, DSC, LP and JORDER-IIF.}
	\vspace{-3mm}
	
	\label{fig:practical}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/p009.tex <==

\def\height{5cm}
\def\name{p9}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/GT_\name.jpg}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name.jpg}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name.jpg}}	\\
			\subfigure[Rain]{
				\includegraphics[width=\height,clip]{./Images/\name/GT_\name_crop.png}}
			\subfigure[ID]{
				\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name_crop.png}}
			\subfigure[CNN]{
				\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name_crop.png}}	\\			
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}   			
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name.jpg}} \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name_crop.png}} 
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name_crop.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/p012.tex <==

\def\height{5cm}
\def\name{p12}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name.jpg}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name.jpg}}
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name.jpg}}	\\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name_crop.png}}
			\subfigure[CNN]{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name_crop.png}}	\\			
	       \subfigure{
	       	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}   			
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name.jpg}} \\
           \subfigure[DSC]{
           	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name_crop.png}} 
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/p019.tex <==

\def\height{5cm}
\def\name{p19}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name.jpg}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name.jpg}}
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name.jpg}}	\\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name_crop.png}}
			\subfigure[CNN]{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name_crop.png}}	\\			
	       \subfigure{
	       	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}   			
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name.jpg}} \\
           \subfigure[DSC]{
           	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name_crop.png}} 
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/rs001.tex <==

\def\height{5.6cm}
\def\name{001}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JORDER]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/rs002.tex <==

\def\height{5.6cm}
\def\name{002}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JORDER]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{002} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/rs003.tex <==

\def\height{5.6cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{003} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/rs004.tex <==

\def\height{5.6cm}
\def\name{004}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{004} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/rs005.tex <==

\def\height{5.6cm}
\def\name{005}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/rs006.tex <==

\def\height{5.6cm}
\def\name{006}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> Trans-Rain Streak Removal_CVPR_arxiv_1126/tex/rs007.tex <==

\def\height{5.6cm}
\def\name{010}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> tex/001.tex <==

\def\height{2.6cm}
\def\name{001}
\def\namet{005}
\def\nameth{008}

\begin{figure*}[htbp]
	\begin{center}
		{ 	
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_001_GT.png}}
            \subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_001_in.png}}
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_ITRI_syn_removal_color_001_in.png}}	
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_DSC_syn_removal_001_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_LP_syn_removal_color_001_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/001/crop_results/crop_Joint-estimated-color-syn-removal-001_in.png}} \\ \vspace{-3mm}		
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/\namet_GT_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/\namet_in_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/ITRI_syn_removal_color_\namet_in_crop.png}}	
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/DSC_syn_removal_\namet_in_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/LP_syn_removal_color_\namet_in_crop.png}}
%			\subfigure{
%				\includegraphics[width=\height,clip]{./Images/\namet/Joint-estimated-color-syn-removal-\namet_in_crop.png}} \\ 
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_008_GT.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_ITRI_syn_removal_color_008_in.png}}	
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_DSC_syn_removal_008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_LP_syn_removal_color_008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/008/crop_results/crop_Joint-estimated-color-syn-removal-008_in.png}} \\			          
		} 
	\end{center}
	\vspace{-3mm}
	\caption{Subjective results of different methods on Rain12. From left to right: Ground truth, rain image, ID, DSC, LP and JORDER. From top to bottom: \textit{Image1} and \textit{Image8}.}
	\vspace{-4mm}
	
	\label{fig:\name}
\end{figure*}


==> tex/002.tex <==

\def\height{5cm}
\def\name{002}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> tex/003.tex <==

\def\height{5cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> tex/004.tex <==

\def\height{5cm}
\def\name{004}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> tex/009.tex <==

\def\height{5cm}
\def\name{009}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in.png}}        
	        \subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in.png}} \\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/\name_in_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_syn_removal_color_\name_in_crop.png}}		
			\subfigure[DSC]{
			\includegraphics[width=\height,clip]{./Images/\name/DSC_syn_removal_\name_in_crop.png}} \\
			\subfigure{
            \includegraphics[width=\height,clip]{./Images/\name/\name_GT.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in.png}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in.png}} \\
           \subfigure[Ground Truth]{
           	\includegraphics[width=\height,clip]{./Images/\name/\name_GT_crop.png}}
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_syn_removal_color_\name_in_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-syn-removal-\name_in_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> tex/blur_case.tex <==

\def\height{5cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-001_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-002_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-003_in.png}}
			\\
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-004_in.png}}			
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-005_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-006_in.png}}
	        \\
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-007_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-009_in.png}}
			\\
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-010_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-011_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/blur_case/Joint-estimated-color-syn-removal-012_in.png}}
		} 
	\end{center}
	\vspace{-2mm}
	\caption{Rain streak removal results on the synthesized blurred images. Blur kernel: Gaussian, whose range is $5\times5$ and blur level $2$.}
	\label{fig:blur_case}
\end{figure*}


==> tex/heavy.tex <==

\def\height{3.6cm}

\begin{figure}[htbp]
	\begin{center}
		{ 	
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/norain-152.png}}
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/rain-152.png}} \\
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-FT-removal-rain-152.png}}	
		\subfigure{
			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-IEF-FT-removal-rain-152.png}}	
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/norain-115.png}}
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/rain-115.png}}
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-FT-removal-rain-115.png}}	
%		\subfigure{
%			\includegraphics[width=\height,clip]{./Images/heavy_cases/SeqRSB-estimated-color-Our-IEF-FT-removal-rain-115.png}}		          
		} 
	\end{center}
	\vspace{-3mm}
	\caption{The results of different methods on the testing image \textit{152} in \textit{Rain100H}.}
	\vspace{-5mm}
	\label{fig:heavy_cases_152}
\end{figure}
\vspace{-2mm}


==> tex/mist_case.tex <==

\def\height{5cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-001_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-002_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-003_in.png}}
			\\
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-004_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-005_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-006_in.png}}
	        \\
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-007_in.png}}
	        \subfigure{
	        	\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-008_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-009_in.png}}
			\\			
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-010_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-011_in.png}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/mist_case/Joint-estimated-color-syn-removal-012_in.png}}
		} 
	\end{center}
	\vspace{-5mm}
	\caption{Rain streak removal results on the synthesized mist images. Fixed transmission: 0.75. Atmospheric light: 0.75.  }
	\label{fig:mist_case}
\end{figure*}


==> tex/p002.tex <==

\def\height{3.7cm}
\def\name{p2}
\def\namet{p19}
\def\nameth{p11}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
			\includegraphics[height=\height,clip]{./Images/\name/GT_\name.jpg}}
			\subfigure{
				\includegraphics[height=\height,clip]{./Images/\namet/GT_\namet.jpg}}
			\subfigure{
				\includegraphics[height=\height,clip]{./Images/\nameth/GT_\nameth.jpg}}
		   \\	
	       \subfigure{
	       	\includegraphics[height=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}
	       \subfigure{
	       	\includegraphics[height=\height,clip]{./Images/\namet/DSC_real_removal_\namet.jpg}}
	       \subfigure{
	       	\includegraphics[height=\height,clip]{./Images/\nameth/DSC_real_removal_\nameth.jpg}}	       
	       \\ 			
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\namet/LP_real_removal_\namet.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\nameth/LP_real_removal_\nameth.jpg}}
           \\
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\name/Joint-estimated-color-Our-FT-removal-Joint-estimated-color-Our-FT-removal-p2.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\namet/Joint-estimated-color-Our-FT-removal-Joint-estimated-color-Our-FT-removal-p19.jpg}}
           \subfigure{
           	\includegraphics[height=\height,clip]{./Images/\nameth/Joint-estimated-color-Our-FT-removal-Joint-estimated-color-Our-FT-removal-p11.jpg}}           
		} 
	\end{center}
	\vspace{-2mm}
	\caption{Subjective results of different methods on real images. From top to down: rain image, DSC, LP and JORDER-IIF.}
	\vspace{-3mm}
	
	\label{fig:practical}
\end{figure*}


==> tex/p009.tex <==

\def\height{5cm}
\def\name{p9}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/GT_\name.jpg}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name.jpg}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name.jpg}}	\\
			\subfigure[Rain]{
				\includegraphics[width=\height,clip]{./Images/\name/GT_\name_crop.png}}
			\subfigure[ID]{
				\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name_crop.png}}
			\subfigure[CNN]{
				\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name_crop.png}}	\\			
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}   			
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
			\subfigure{
				\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name.jpg}} \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name_crop.png}} 
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name_crop.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> tex/p012.tex <==

\def\height{5cm}
\def\name{p12}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name.jpg}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name.jpg}}
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name.jpg}}	\\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name_crop.png}}
			\subfigure[CNN]{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name_crop.png}}	\\			
	       \subfigure{
	       	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}   			
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name.jpg}} \\
           \subfigure[DSC]{
           	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name_crop.png}} 
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> tex/p019.tex <==

\def\height{5cm}
\def\name{p19}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name.jpg}}
	        \subfigure{
	        \includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name.jpg}}
			\subfigure{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name.jpg}}	\\
            \subfigure[Rain]{
			\includegraphics[width=\height,clip]{./Images/\name/GT_\name_crop.png}}
			\subfigure[ID]{
			\includegraphics[width=\height,clip]{./Images/\name/ITRI_real_removal_color_\name_crop.png}}
			\subfigure[CNN]{
			\includegraphics[width=\height,clip]{./Images/\name/NNRestore_real_removal_\name_crop.png}}	\\			
	       \subfigure{
	       	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name.jpg}}   			
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name.jpg}}
           \subfigure{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name.jpg}} \\
           \subfigure[DSC]{
           	\includegraphics[width=\height,clip]{./Images/\name/DSC_real_removal_\name_crop.png}} 
           \subfigure[LP]{
           	\includegraphics[width=\height,clip]{./Images/\name/LP_real_removal_\name_crop.png}}
           \subfigure[JODAR]{
           	\includegraphics[width=\height,clip]{./Images/\name/Joint-estimated-color-real-removal-\name_crop.png}} \\		
		} 
	\end{center}
	\vspace{-5mm}
	\caption{}
	\label{fig:\name}
\end{figure*}


==> tex/rs001.tex <==

\def\height{5.6cm}
\def\name{001}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JORDER]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> tex/rs002.tex <==

\def\height{5.6cm}
\def\name{002}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JORDER]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{002} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> tex/rs003.tex <==

\def\height{5.6cm}
\def\name{003}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{003} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> tex/rs004.tex <==

\def\height{5.6cm}
\def\name{004}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{004} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> tex/rs005.tex <==

\def\height{5.6cm}
\def\name{005}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> tex/rs006.tex <==

\def\height{5.6cm}
\def\name{006}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}


==> tex/rs007.tex <==

\def\height{5.6cm}
\def\name{010}

\begin{figure*}[!htbp]
	\begin{center}
		{ 	\subfigure[Input]{
            \includegraphics[width=\height,clip]{./Images/\name/\name_in.png}}
	        \subfigure[ID]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/ITRI_syn_rain_streak_\name_in.png}}
	        \subfigure[CNN]{
	        	\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/NNRestore_syn_rain_streak_\name_in.png}}
	        \\
			\subfigure[DSC]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/DSC_syn_rain_streak_\name_in.png}}
			\subfigure[LP]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/LP_syn_rain_streak_\name_in.png}}
			\subfigure[JODAR]{
				\includegraphics[width=\height,clip]{./Images/Syn_Rain_Streak/Joint-estimated-syn-rain-level-\name_in.png}}		
		} 
	\end{center}
	\caption{Rain Streaks of different methods on the testing image \textit{001} in \textit{Rain12}.}
	\label{fig:\name}
\end{figure*}

